Generating Query Focused Summaries from Query-Free Resources

The availability of large-scale datasets has driven the development of neural models that create generic summaries from single or multiple documents. In this work we consider query focused summarization (QFS), a task for which training data in the form of queries, documents, and summaries is not readily available. We propose to decompose QFS into (1) query modeling (i.e., finding supportive evidence within a set of documents for a query) and (2) conditional language modeling (i.e., summary generation). We introduce MaRGE, a Masked ROUGE Regression framework for evidence estimation and ranking which relies on a unified representation for summaries and queries, so that summaries in generic data can be converted into proxy queries for learning a query model. Experiments across QFS benchmarks and query types show that our model achieves state-of-the-art performance despite learning from weak supervision.

==> tab_evidence.tex <==
\begin{table*}[t]
% \tabcolsep=0.1cm
\bgroup
\def\arraystretch{1.0}
\centerline{
% \begin{small}
\begin{tabular}{@{}l@{~}@{~}c@{~~}c@{~~}cc@{~~}c@{~~}c@{}}  % The first row
\hline
\multirow{2}*{\textbf{Models}} 
& \multicolumn{3}{c}{\textbf{DUC 2006}} 
& \multicolumn{3}{c}{\textbf{DUC 2007}}\\
~ & {R-1} & {R-2} & {R-SU4} & {R-1} & {R-2} & {R-SU4} \\
\hline
{\sc TermFreq}\\
{\sc  BertQa}
&38.6 &\hspace*{.8ex}8.4	&13.9	&39.8	&10.0	&14.9\\
{\sc  BertMrc}\\
% {\sc  IR+BertQa}
% &39.2	&\hspace*{.8ex}8.6	&14.2
% &41.7	&10.9	&15.9\\
\hline
{\sc  MaskAll}$^\dagger$ & 34.2	&\hspace*{.8ex}6.5	&11.6&	37.9&	\hspace*{1.2ex}8.6 &	13.7\\
{\sc  NoMask}$^\dagger$ & 38.3	&\hspace*{.8ex}8.0	&13.7 & 40.3	&10.0	&15.4\\
{\sc  RandMask}$^\dagger$ \\
\hline
{\sc  Marge-Mn$^\dagger$}
&{39.0}	&\hspace*{.8ex}\bf{9.3}&	{14.5}	&{41.6}	&\bf{11.6}&	{16.6}\\
{\hspace*{2.2ex}-Verbs}
&38.4	&\hspace*{0.8ex}8.9&	14.0&	41.5&	11.4&	16.3\\
{\sc  Marge-Cd$^\dagger$}
&38.4   &\hspace*{.8ex}8.6&	13.9
&40.7   &10.8&	15.8\\
{\sc  MargeFs$^\dagger$}
&\bf{39.5}	&\hspace*{0.8ex}9.2	&\bf{14.7}
&\bf{42.4}	&\bf{11.6}	&\bf{16.8}\\
\hline
\end{tabular}
% \end{small}
}
\egroup
\caption{\label{tab:evidence_duc} 
  Performance of content selectors on DUC 2006 and 2007. 
  R-1, R-2 and R-SU4 stand for the F1 score of ROUGE~1, 2, and SU4, respectively. Models with $\dagger$ are proposed in this work.
}
\end{table*}

==> tab_fs.tex <==
\begin{table*}[t]
% \tabcolsep=0.05cm
\bgroup
\def\arraystretch{1.0}
\centerline{
% \begin{small}
% \begin{tabular}{@{}l@{~}@{~}c@{~~}c@{~~}cc@{~~}c@{~~}c@{}}
\begin{tabular}{lccc ccc ccc}
\hline
\multirow{2}*{\textbf{Models}} 
& \multicolumn{3}{c}{\textbf{DUC 2006}} 
& \multicolumn{3}{c}{\textbf{DUC 2007}}
& \multicolumn{3}{c}{\textbf{TD-QFS}}\\
~ & {R-1} & {R-2} & {R-SU4} 
& {R-1} & {R-2} & {R-SU4} 
& {R-1} & {R-2} & {R-SU4}\\
\hline
{\sc  Marge-Mn$^\dagger$}
&{39.0}	&\hspace*{.8ex}\bf{9.3}&	{14.5}	&{41.6}	&\bf{11.6}&	{16.6}\\
{\sc  MargeFs-Mn$^\dagger$}
&\bf{39.5}	&\hspace*{0.8ex}9.2	&\bf{14.7}
&\bf{42.4}	&\bf{11.6}	&\bf{16.8}\\
\hline
{\sc  Marge-CnnDm$^\dagger$}
&38.4   &\hspace*{.8ex}8.6&	13.9
&40.7   &10.8&	15.8\\
{\sc  MargeFs-CnnDm$^\dagger$}\\
\hline
\end{tabular}
}
\egroup
\caption{\label{tab:ext_duc} 
  Performance of content selectors on QFS. 
  R-1, R-2 and R-SU4 stand for the F1 score of ROUGE~1, 2, and SU4, respectively. Systems with $\dagger$ are proposed in this work.
}
\end{table*}


==> tab_mn_example.tex <==
\begin{table*}[t]
% \fontsize{11}{4}\selectfont
\scriptsize
% \centering
\bgroup
\def\arraystretch{1.0}
\centering
\begin{tabular}{@{~}p{16cm}@{~}}\hline
% \textbf{Query title}: Crime and Law Enforcement in China
% \\\hline
% ggreen, gblue, gyellow, gred
\textbf{Query}: Computer viruses. Identify computer viruses detected worldwide. Include such details as how they are spread, what operating systems they affect, what damage they inflict, their country of origin, and their creators wherever possible.
\\\hline
\textbf{\textsc{MargeSum-Mn}}: 
The FBI is trying to track the author of a file - destroying computer virus that has hit some of the nation's biggest corporations and infected tens of thousands of machines, \textbf{\textcolor{gblue}{the AP reports.}} 
According to South Africa's computer virus helpline co-ordinator Ian Melamed, Hare Krsna is at present the most widely reported computer virus in the country and could wipe out all information stored on the hard drives of infected computers on that date.
The new virus, named W32/KRIZ.3862, is designed to damage Windows 95, Windows 98, and Windows NT machines. 
\textbf{\textcolor{gblue}{Xinhua reports}} that the Philippine government asked the congress Tuesday to pass a law that would impose stiff penalties on cyber crimes following a delay in the arrest of the suspected creators of the "love bug" computer virus. 
The virus, which was allegedly created by a Philippine couple using internet access cards, has caused up to 2.6 billion dollars in damage to computer systems in more than 20 countries in Asia, America, and Europe, an expert at Carnegie Mellon University \textbf{\textcolor{gblue}{tells the AP}}. 
Home-made computer viruses are not new in Bangladesh, as the country's first locally-produced virus, the Dhaka virus, was created in 1991. 
Experts say off-the-shelf the antivirus software can prevent infection. 
\textbf{\textcolor{gblue}{The AP notes}} that the virus is only known to attack computers using Microsoft's Word 97 or Word 2000 programs, but experts say it's not as effective as the original.
 \\\hdashline
\textbf{\textsc{MargeSum-Mn}+Query}: 
\textbf{\textcolor{ggreen}{Here's what you need to know about computer viruses detected worldwide. Include such details as how they are spread, the operating systems they affect, their country of origin, and their creators of the virus ver possible.}}
\textbf{\textcolor{gred}{Click here to read the full list of computer viruses, including the number of cases they are spreading, the damage they inflict, their state of origin and their country's country of origins, and the amount of damage ver has done to computer systems in more than 20 countries in Asia, America, and Europe}, \textcolor{gblue}{the AP reports}}. 
\textbf{\textcolor{gblue}{The AP quotes}} an expert at Carnegie Mellon University as saying Hare Krsna is at present the most widely reported computer virus in the country and could wipe out all information stored on the hard drives of infected computers on Christmas day, a potential security breach that should worry businesses and governments, an expert said Saturday, \textbf{\textcolor{gblue}{per Xinhua,}} which notes that the FBI on Friday tried to track the author of a computer - destroying computer virus that has hit some of the nation's biggest corporations and infected tens of thousands of machines, \textbf{\textcolor{gblue}{per the AP.}}
\textbf{\textcolor{gred}{(Click to read about the Chernobyl virus, or to see how it could be used to wipe out information on hard drives without warning ) ...}}
But it's the most widespread computer virus ever reported in South Africa, according to South Africa's computer virus helpline co-ordinator Ian Melamed, who says the virus is "the most commonly reported" computer virus.
\\\hline
\end{tabular}
\caption{\label{tab:mn_example}
System outputs for cluster D0629B in DUC 2006.
We show three dataset-specific summary patterns of Multi-News that can harm QFS performance: 
1) \textbf{\textcolor{gblue}{extra press information}}, 
2) \textbf{\textcolor{ggreen}{lazy query copy}} and 
3) \textbf{\textcolor{gred}{hallucinating hyperlink}} (better view in color). 
}
\egroup
\end{table*}
%\end{minipage}
%\end{multicols}

